Existence of Noise Induced Order, a Computer Aided Proof

We prove the existence of Noise Induced Order in the Matsumoto-Tsuda model, where it was originally discovered in 1983 by numerical simulations. This is a model of the famous Belosouv-Zabotinsky reaction, a chaotic chemical reaction, and consists of a one dimensional random dynamical system with additive noise. The simulations showed that an increase in amplitude of the noise causes the Lyapunov exponent to decrease from positive to negative; we give a mathematical proof of the existence of this transition. The method we use relies on some computer aided estimates providing a certified approximation of the stationary measure in the $L^{1}$ norm. This is realized by explicit functional analytic estimates working together with an efficient algorithm. The method is general enough to be adapted to any piecewise differentiable dynamical system on the unit interval with additive noise. We also prove that the stationary measure of the system varies in a Lipschitz way if the system is perturbed and that the Lyapunov exponent of the system varies in a H\"older way when the noise amplitude increases.

==> data_sheet.tex <==
noise	delta_contr	alpha_contr	n_contr	delta	alpha	sumCi	l1apriori	delta_est	l1err	lyap
$0.860\times 10^{-2} $ & $2^{-18}$ & $0.023$ & $56$ & $2^{-27}$ & $0.044$ & $29.54$ & $0.445\times 10^{-4} $ & $2^{-14}$ & $0.246\times 10^{-5} $ & $-6.03^{536}_{602}\times 10^{-1} $\\ 
$0.785\times 10^{-2} $ & $2^{-18}$ & $0.017$ & $58$ & $2^{-27}$ & $0.039$ & $29.20$ & $0.479\times 10^{-4} $ & $2^{-14}$ & $0.257\times 10^{-5} $ & $-5.499^{221}_{901}\times 10^{-1} $\\ 
$0.721\times 10^{-2} $ & $2^{-18}$ & $0.013$ & $60$ & $2^{-27}$ & $0.037$ & $28.95$ & $0.517\times 10^{-4} $ & $2^{-14}$ & $0.268\times 10^{-5} $ & $-4.985^{026}_{749}\times 10^{-1} $\\ 
$0.661\times 10^{-2} $ & $2^{-18}$ & $0.015$ & $60$ & $2^{-27}$ & $0.04$ & $28.75$ & $0.562\times 10^{-4} $ & $2^{-14}$ & $0.282\times 10^{-5} $ & $-4.467^{104}_{862}\times 10^{-1} $\\ 
$0.606\times 10^{-2} $ & $2^{-18}$ & $0.022$ & $54$ & $2^{-27}$ & $0.05$ & $28.44$ & $0.612\times 10^{-4} $ & $2^{-14}$ & $0.296\times 10^{-5} $ & $-3.95^{558}_{636}\times 10^{-1} $\\ 
$0.556\times 10^{-2} $ & $2^{-18}$ & $0.015$ & $58$ & $2^{-27}$ & $0.046$ & $28.77$ & $0.672\times 10^{-4} $ & $2^{-14}$ & $0.311\times 10^{-5} $ & $-3.462^{063}_{884}\times 10^{-1} $\\ 
$0.509\times 10^{-2} $ & $2^{-18}$ & $0.014$ & $60$ & $2^{-27}$ & $0.048$ & $29.19$ & $0.747\times 10^{-4} $ & $2^{-14}$ & $0.330\times 10^{-5} $ & $-2.97^{272}_{360}\times 10^{-1} $\\ 
$0.466\times 10^{-2} $ & $2^{-18}$ & $0.019$ & $59$ & $2^{-27}$ & $0.056$ & $29.56$ & $0.832\times 10^{-4} $ & $2^{-14}$ & $0.351\times 10^{-5} $ & $-2.52^{476}_{568}\times 10^{-1} $\\ 
$0.426\times 10^{-2} $ & $2^{-18}$ & $0.032$ & $53$ & $2^{-27}$ & $0.072$ & $29.70$ & $0.930\times 10^{-4} $ & $2^{-14}$ & $0.374\times 10^{-5} $ & $-2.10^{322}_{419}\times 10^{-1} $\\ 
$0.391\times 10^{-2} $ & $2^{-18}$ & $0.025$ & $57$ & $2^{-27}$ & $0.07$ & $30.68$ & $0.104\times 10^{-3} $ & $2^{-14}$ & $0.400\times 10^{-5} $ & $-1.74^{370}_{474}\times 10^{-1} $\\ 
$0.359\times 10^{-2} $ & $2^{-18}$ & $0.023$ & $60$ & $2^{-27}$ & $0.074$ & $31.73$ & $0.118\times 10^{-3} $ & $2^{-14}$ & $0.431\times 10^{-5} $ & $-1.42^{733}_{844}\times 10^{-1} $\\ 
$0.329\times 10^{-2} $ & $2^{-18}$ & $0.028$ & $60$ & $2^{-27}$ & $0.085$ & $32.63$ & $0.134\times 10^{-3} $ & $2^{-14}$ & $0.467\times 10^{-5} $ & $-1.1^{588}_{600}\times 10^{-1} $\\ 
$0.302\times 10^{-2} $ & $2^{-18}$ & $0.034$ & $60$ & $2^{-27}$ & $0.097$ & $33.55$ & $0.152\times 10^{-3} $ & $2^{-14}$ & $0.510\times 10^{-5} $ & $-9.^{399}_{411}\times 10^{-2} $\\ 
$0.277\times 10^{-2} $ & $2^{-18}$ & $0.044$ & $58$ & $2^{-27}$ & $0.11$ & $34.26$ & $0.173\times 10^{-3} $ & $2^{-14}$ & $0.560\times 10^{-5} $ & $-7.^{692}_{706}\times 10^{-2} $\\ 
$0.252\times 10^{-2} $ & $2^{-18}$ & $0.053$ & $56$ & $2^{-27}$ & $0.13$ & $35.04$ & $0.198\times 10^{-3} $ & $2^{-14}$ & $0.626\times 10^{-5} $ & $-6.3^{035}_{187}\times 10^{-2} $\\ 
$0.232\times 10^{-2} $ & $2^{-18}$ & $0.053$ & $56$ & $2^{-27}$ & $0.14$ & $35.94$ & $0.223\times 10^{-3} $ & $2^{-14}$ & $0.693\times 10^{-5} $ & $-5.4^{305}_{472}\times 10^{-2} $\\ 
$0.212\times 10^{-2} $ & $2^{-18}$ & $0.055$ & $56$ & $2^{-27}$ & $0.15$ & $36.88$ & $0.254\times 10^{-3} $ & $2^{-14}$ & $0.784\times 10^{-5} $ & $-4.7^{769}_{957}\times 10^{-2} $\\ 
$0.192\times 10^{-2} $ & $2^{-18}$ & $0.051$ & $58$ & $2^{-27}$ & $0.16$ & $38.21$ & $0.293\times 10^{-3} $ & $2^{-14}$ & $0.909\times 10^{-5} $ & $-4.3^{776}_{993}\times 10^{-2} $\\ 
$0.177\times 10^{-2} $ & $2^{-18}$ & $0.053$ & $58$ & $2^{-27}$ & $0.18$ & $38.98$ & $0.329\times 10^{-3} $ & $2^{-14}$ & $0.104\times 10^{-4} $ & $-4.2^{654}_{897}\times 10^{-2} $\\ 
$0.162\times 10^{-2} $ & $2^{-18}$ & $0.054$ & $58$ & $2^{-27}$ & $0.19$ & $39.82$ & $0.373\times 10^{-3} $ & $2^{-14}$ & $0.121\times 10^{-4} $ & $-4.3^{194}_{479}\times 10^{-2} $\\ 
$0.150\times 10^{-2} $ & $2^{-18}$ & $0.055$ & $58$ & $2^{-27}$ & $0.2$ & $40.53$ & $0.419\times 10^{-3} $ & $2^{-14}$ & $0.139\times 10^{-4} $ & $-4.^{488}_{521}\times 10^{-2} $\\ 
$0.137\times 10^{-2} $ & $2^{-18}$ & $0.063$ & $57$ & $2^{-27}$ & $0.23$ & $41.00$ & $0.476\times 10^{-3} $ & $2^{-14}$ & $0.164\times 10^{-4} $ & $-4.7^{613}_{992}\times 10^{-2} $\\ 
$0.125\times 10^{-2} $ & $2^{-18}$ & $0.066$ & $58$ & $2^{-27}$ & $0.25$ & $42.14$ & $0.554\times 10^{-3} $ & $2^{-14}$ & $0.200\times 10^{-4} $ & $-5.1^{293}_{750}\times 10^{-2} $\\ 
$0.115\times 10^{-2} $ & $2^{-18}$ & $0.071$ & $58$ & $2^{-27}$ & $0.27$ & $43.12$ & $0.636\times 10^{-3} $ & $2^{-14}$ & $0.239\times 10^{-4} $ & $-5.^{491}_{545}\times 10^{-2} $\\ 
$0.105\times 10^{-2} $ & $2^{-18}$ & $0.079$ & $58$ & $2^{-27}$ & $0.3$ & $44.28$ & $0.747\times 10^{-3} $ & $2^{-14}$ & $0.294\times 10^{-4} $ & $-5.9^{172}_{835}\times 10^{-2} $\\ 
$0.960\times 10^{-3} $ & $2^{-18}$ & $0.086$ & $58$ & $2^{-27}$ & $0.34$ & $45.41$ & $0.876\times 10^{-3} $ & $2^{-14}$ & $0.360\times 10^{-4} $ & $-6.^{346}_{427}\times 10^{-2} $\\ 
$0.885\times 10^{-3} $ & $2^{-18}$ & $0.092$ & $58$ & $2^{-27}$ & $0.37$ & $46.43$ & $0.102\times 10^{-2} $ & $2^{-14}$ & $0.436\times 10^{-4} $ & $-6.^{758}_{855}\times 10^{-2} $\\ 
$0.810\times 10^{-3} $ & $2^{-18}$ & $0.095$ & $58$ & $2^{-27}$ & $0.4$ & $47.44$ & $0.119\times 10^{-2} $ & $2^{-14}$ & $0.534\times 10^{-4} $ & $-7.^{200}_{320}\times 10^{-2} $\\ 
$0.748\times 10^{-3} $ & $2^{-18}$ & $0.098$ & $58$ & $2^{-27}$ & $0.43$ & $48.25$ & $0.138\times 10^{-2} $ & $2^{-14}$ & $0.643\times 10^{-4} $ & $-7.^{569}_{711}\times 10^{-2} $\\ 
$0.686\times 10^{-3} $ & $2^{-18}$ & $0.1$ & $57$ & $2^{-27}$ & $0.46$ & $48.65$ & $0.162\times 10^{-2} $ & $2^{-14}$ & $0.779\times 10^{-4} $ & $-^{7.888}_{8.061}\times 10^{-2} $\\ 
$0.623\times 10^{-3} $ & $2^{-18}$ & $0.099$ & $56$ & $2^{-27}$ & $0.5$ & $49.04$ & $0.192\times 10^{-2} $ & $2^{-14}$ & $0.956\times 10^{-4} $ & $-8.^{068}_{280}\times 10^{-2} $\\ 
$0.573\times 10^{-3} $ & $2^{-19}$ & $0.07$ & $60$ & $2^{-27}$ & $0.29$ & $46.78$ & $0.141\times 10^{-2} $ & $2^{-15}$ & $0.595\times 10^{-4} $ & $-8.^{076}_{209}\times 10^{-2} $\\ 
$0.524\times 10^{-3} $ & $2^{-19}$ & $0.085$ & $56$ & $2^{-27}$ & $0.33$ & $46.32$ & $0.162\times 10^{-2} $ & $2^{-15}$ & $0.696\times 10^{-4} $ & $-7.^{784}_{940}\times 10^{-2} $\\ 
$0.480\times 10^{-3} $ & $2^{-19}$ & $0.07$ & $58$ & $2^{-27}$ & $0.34$ & $47.75$ & $0.185\times 10^{-2} $ & $2^{-15}$ & $0.800\times 10^{-4} $ & $-7.^{312}_{490}\times 10^{-2} $\\ 
$0.436\times 10^{-3} $ & $2^{-19}$ & $0.066$ & $58$ & $2^{-27}$ & $0.36$ & $48.66$ & $0.215\times 10^{-2} $ & $2^{-15}$ & $0.935\times 10^{-4} $ & $-6.^{653}_{861}\times 10^{-2} $\\ 
$0.399\times 10^{-3} $ & $2^{-19}$ & $0.06$ & $60$ & $2^{-27}$ & $0.39$ & $50.39$ & $0.254\times 10^{-2} $ & $2^{-15}$ & $0.110\times 10^{-3} $ & $-^{5.964}_{6.208}\times 10^{-2} $\\ 
$0.368\times 10^{-3} $ & $2^{-19}$ & $0.065$ & $60$ & $2^{-27}$ & $0.43$ & $51.36$ & $0.299\times 10^{-2} $ & $2^{-15}$ & $0.128\times 10^{-3} $ & $-5.^{339}_{623}\times 10^{-2} $\\ 
$0.343\times 10^{-3} $ & $2^{-20}$ & $0.041$ & $65$ & $2^{-27}$ & $0.24$ & $49.27$ & $0.232\times 10^{-2} $ & $2^{-16}$ & $0.976\times 10^{-4} $ & $-^{4.871}_{5.086}\times 10^{-2} $\\ 
$0.312\times 10^{-3} $ & $2^{-20}$ & $0.044$ & $65$ & $2^{-27}$ & $0.26$ & $50.33$ & $0.270\times 10^{-2} $ & $2^{-16}$ & $0.112\times 10^{-3} $ & $-4.^{189}_{436}\times 10^{-2} $\\ 
$0.287\times 10^{-3} $ & $2^{-20}$ & $0.048$ & $65$ & $2^{-27}$ & $0.29$ & $51.29$ & $0.309\times 10^{-2} $ & $2^{-16}$ & $0.127\times 10^{-3} $ & $-3.^{565}_{844}\times 10^{-2} $\\ 
$0.259\times 10^{-3} $ & $2^{-20}$ & $0.042$ & $67$ & $2^{-27}$ & $0.31$ & $53.14$ & $0.368\times 10^{-2} $ & $2^{-16}$ & $0.149\times 10^{-3} $ & $-2.^{659}_{984}\times 10^{-2} $\\ 
$0.237\times 10^{-3} $ & $2^{-20}$ & $0.046$ & $67$ & $2^{-27}$ & $0.35$ & $54.32$ & $0.431\times 10^{-2} $ & $2^{-17}$ & $0.144\times 10^{-3} $ & $-1.^{686}_{998}\times 10^{-2} $\\ 
$0.218\times 10^{-3} $ & $2^{-20}$ & $0.05$ & $67$ & $2^{-27}$ & $0.38$ & $55.49$ & $0.504\times 10^{-2} $ & $2^{-17}$ & $0.165\times 10^{-3} $ & $-^{5.731}_{9.274}\times 10^{-3} $\\ 
$0.199\times 10^{-3} $ & $2^{-20}$ & $0.051$ & $68$ & $2^{-27}$ & $0.42$ & $57.28$ & $0.606\times 10^{-2} $ & $2^{-17}$ & $0.193\times 10^{-3} $ & $^{7.138}_{2.988}\times 10^{-3} $\\ 
$0.184\times 10^{-3} $ & $2^{-20}$ & $0.051$ & $69$ & $2^{-27}$ & $0.46$ & $59.07$ & $0.725\times 10^{-2} $ & $2^{-17}$ & $0.225\times 10^{-3} $ & $1.^{844}_{362}\times 10^{-2} $\\ 
$0.168\times 10^{-3} $ & $2^{-20}$ & $0.053$ & $70$ & $2^{-27}$ & $0.5$ & $61.10$ & $0.896\times 10^{-2} $ & $2^{-17}$ & $0.272\times 10^{-3} $ & $2.^{977}_{394}\times 10^{-2} $\\ 
$0.154\times 10^{-3} $ & $2^{-21}$ & $0.042$ & $74$ & $2^{-27}$ & $0.29$ & $57.78$ & $0.650\times 10^{-2} $ & $2^{-18}$ & $0.708\times 10^{-4} $ & $3.^{689}_{533}\times 10^{-2} $\\ 
$0.142\times 10^{-3} $ & $2^{-21}$ & $0.048$ & $74$ & $2^{-27}$ & $0.32$ & $59.11$ & $0.757\times 10^{-2} $ & $2^{-18}$ & $0.822\times 10^{-4} $ & $4.^{462}_{282}\times 10^{-2} $\\ 
$0.129\times 10^{-3} $ & $2^{-21}$ & $0.049$ & $75$ & $2^{-27}$ & $0.36$ & $60.98$ & $0.901\times 10^{-2} $ & $2^{-18}$ & $0.988\times 10^{-4} $ & $5.^{239}_{023}\times 10^{-2} $\\ 
$0.117\times 10^{-3} $ & $2^{-21}$ & $0.054$ & $75$ & $2^{-27}$ & $0.4$ & $62.70$ & $0.110\times 10^{-1} $ & $2^{-18}$ & $0.123\times 10^{-3} $ & $^{6.093}_{5.823}\times 10^{-2} $\\ 
$0.106\times 10^{-3} $ & $2^{-21}$ & $0.058$ & $75$ & $2^{-27}$ & $0.45$ & $64.34$ & $0.135\times 10^{-1} $ & $2^{-18}$ & $0.154\times 10^{-3} $ & $6.^{965}_{626}\times 10^{-2} $\\ 
$0.966\times 10^{-4} $ & $2^{-21}$ & $0.06$ & $75$ & $2^{-27}$ & $0.49$ & $65.89$ & $0.165\times 10^{-1} $ & $2^{-18}$ & $0.193\times 10^{-3} $ & $7.^{851}_{428}\times 10^{-2} $\\ 
$0.873\times 10^{-4} $ & $2^{-21}$ & $0.062$ & $75$ & $2^{-27}$ & $0.55$ & $67.55$ & $0.209\times 10^{-1} $ & $2^{-18}$ & $0.252\times 10^{-3} $ & $8.^{917}_{365}\times 10^{-2} $\\ 


==> nio_section5b.tex <==

%\begin{document}



\label{algsec}

We provide here an overview of the main algorithm in pseudo-code. The
description of the functions that appear in the algorithm follows,
complemented with necessary references to the mathematical part.

\begin{algorithm}[H]
  \caption{\emph{MainAlgorithm}, invokes other algorithms and returns an in interval
    enclosing rigorously the Lyapunov exponent.  }
\begin{algorithmic}
  \REQUIRE $\xi$ \COMMENT{noise size},\\
  $\delta$ \COMMENT{the partition size of the approximation of the invariant measure}, \\
  $\delta_{\textrm{contr}}$ \COMMENT{coarser size used estimating the contraction rate,
    multiple of $\delta$},\\
  $\delta_{\textrm{est}}$ \COMMENT{coarser size used estimating measure's
    error, multiple of $\delta$}.\\
  \ENSURE $\lambda$ \COMMENT{interval enclosing the Lyapunov exponent}.  \algrule \STATE
  $L_{\delta_{\textrm{contr}},\xi} \gets Matrix(\pi_{\delta_{\textrm{contr}}}\cdot
  N_{\xi}\cdot\pi_{\delta_{\textrm{contr}}}\cdot L\cdot\pi_{\delta_{\textrm{contr}}})$
  \STATE
  $\alpha_{\textrm{contr}},\overline{n}_{\textrm{contr}},(C_{i,\textrm{contr}})_{1\leq i\leq\overline{n}} \gets
  EstimateContractionRate(L_{\delta_{\textrm{contr}},\xi})$
  \STATE
  $L_{\delta,\xi} \gets Matrix(\pi_{\delta}\cdot N_{\xi}\cdot\pi_{\delta}\cdot
  L\cdot\pi_{\delta})$
  \STATE
  $\alpha,\overline{n},(C_{i})_{1\leq i\leq\overline{n}} \gets
  CoarseFineEstimate(\alpha_{\textrm{contr}},\overline{n}_{\textrm{contr}},(C_{i,\textrm{contr}})_{1\leq
    i\leq\overline{n}})$
  \STATE
  $\tilde{f},numericError \gets RigorousFixedPoint(L_{\delta,\xi})$
  \STATE $\Pi_{\textrm{est}} \gets UniformPartition(\delta_{\textrm{est}})$ \STATE
  $L1ErrorBound \gets ComputeL1ErrorBound(\Pi_{\textrm{est}},\alpha,\overline{n},(C_i)_{1\leq
    i\leq\overline{n}},\tilde{f},numericError)$
  \STATE $LInfBound[I] \gets ComputeLInfinityBound(\Pi_{\textrm{est}},\tilde{f})$ \STATE
  $\lambda \gets RigorousObservableEstimation(log|T'|, \tilde{f}, L1ErrorBound,
  LInfBound[I])$ \RETURN $\lambda$
\end{algorithmic}
\end{algorithm}

Here is the explanation of the functions being used:

\begin{itemize}
\item \emph{Matrix} function, computes with rigorous precision the matrix
representing the finite dimensional approximation of an operator acting on a
finite dimensional space.

\item \emph{EstimateContractionRate} function, for a certain $\delta_{\text{%
contr}}$ ($>\delta$), computes suitable $\alpha_{\text{contr}}$ and $%
\overline{n}_{\text{contr}}$, and gives as byproduct $C_{i,\text{contr}}$,
that is a bound for $||L_{\delta_{\text{contr}},\xi
}^{i}|_V||_{L^{1}\rightarrow L^{1}}$ for $1\leq i <\overline{n}_{\text{contr}%
}$. Needless to say, in practice this procedure may fail, if unable to
detect any contraction in a reasonable time. In the cases under
consideration we obtain a suitable contraction (with $\alpha_{\text{contr}%
}\leq 0.1$, that will yield $\alpha\leq 0.6$) for $\overline{n}_{\text{contr}%
}\approx 60$.

\item \emph{CoarseFineEstimate} function applied the coarse-fine process
explained in Section \ref{coarsefine}, to obtain a bound $\alpha$ on $%
||L_{\delta ,\xi }^{i}|_V||_{L^{1}\rightarrow L^{1}}$ for the real $\delta$,
from the computed $\alpha_{\text{contr}}$ estimating $||L_{\delta_{\text{%
contr}},\xi }^{i}|_V||_{L^{1}\rightarrow L^{1}}$ for a bigger $\delta_{\text{%
contr}}$, as explained in Section \ref{coarsefine}.

\item \emph{RigorousFixedPoint} function, computes the vector that is fixed
my a matrix, and returns the rigorous numerical error, this function is used
as a blackbox from numerical algebra.

\item \emph{ComputeL1ErrorBound} function, estimates the error in the
approximation of the invariant measure applying all the techniques explained
in Section \ref{firstalgo}.

\item \emph{ComputeLInfinityBound} function, computes a bound on the $%
L^\infty$ norm of the density in the interval of a certain partition, as
explained in Subsection \ref{LocLInfty}.

\item \emph{RigorousObservableEstimation} function, estimates rigorously the
integral of an observable, as explained in Section \ref{Lyap}.
\end{itemize}


%\end{document}

==> nio_section8.tex <==

\label{toy}

Let us consider the continuous map $T:[0,1]\rightarrow \lbrack 0,1]$ defined
as 
\begin{equation*}
T(x)=\left\{ 
\begin{array}{cc}
2x & 0\leq x \leq {1}{4} \\ 
-2(x-\frac{1}{2}) & \frac{1}{4}\leq x\leq \frac{1}{2} \\ 
0 & \frac{1}{2}\leq x\leq 1.%
\end{array}%
\right.
\end{equation*}
whose graph is represented in Figure \ref{f1}. 
\begin{figure}[htbp]
\centering
\includegraphics[height=3cm, width=5cm]{Toy_Model.png}
\caption{The map $T$.}
\label{f1}
\end{figure}
Notice that the interval $[\frac{1}{2},1]$ is sent to $0$ by the map. Since
the map send the interval $[0,\frac12]$ to itself, the system has an
absolutely continuous invariant measure which is also a physical measure
(the basin has positive Lebesgue measure) $\mu =2m $, where $m$ is the
Lebesgue measure on $[0,\frac{1}{2}]$. Let again $L$ be the transfer
operator associated to $T$. If we now add a small noise and consider $N_{\xi
}L$ this operator will still have an absolutely continuous invariant measure 
$\mu _{\xi }$. Now $\mu _{\xi }([\frac{1}{2},1])>0$, and then the Lyapunov
exponent of the system with noise is $-\infty $. This is quite a
caricatural, extreme version of the system studied in Section \ref{map}.
Interesting, intermediate versions can be constructed by replacing the
constant ``$0$'' branch of $T$ in the interval $[\frac{1}{2},1]$ with a map $%
g\in C^{2}$ such that: $g(\frac{1}{2})=0$, $g(1)=0$, $||g^{\prime
}||_{\infty }\leq \epsilon $ for some small $\epsilon $.
We refer to \cite{D} for a somewhat similar example.
